Image-based Deep Learning for Smart Digital Twins: a Review

Smart Digital twins (SDTs) are being increasingly used to virtually replicate and predict the behaviors of complex physical systems through continual data assimilation enabling the optimization of the performance of these systems by controlling the actions of systems. Recently, deep learning (DL) models have significantly enhanced the capabilities of SDTs, particularly for tasks such as predictive maintenance, anomaly detection, and optimization. In many domains, including medicine, engineering, and education, SDTs use image data (image-based SDTs) to observe and learn system behaviors and control their behaviors. This paper focuses on various approaches and associated challenges in developing image-based SDTs by continually assimilating image data from physical systems. The paper also discusses the challenges involved in designing and implementing DL models for SDTs, including data acquisition, processing, and interpretation. In addition, insights into the future directions and opportunities for developing new image-based DL approaches to develop robust SDTs are provided. This includes the potential for using generative models for data augmentation, developing multi-modal DL models, and exploring the integration of DL with other technologies, including 5G, edge computing, and IoT. In this paper, we describe the image-based SDTs, which enable broader adoption of the digital twin DT paradigms across a broad spectrum of areas and the development of new methods to improve the abilities of SDTs in replicating, predicting, and optimizing the behavior of complex systems.

==> tex/IEEEbiography.tex <==
% \vspace{-2.5em}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/peggy.jpg}}]{Pei-Chi Huang} received the Ph.D. degree from the University of Texas at Austin, Texas, USA, in 2017. She is currently an assistant professor with the Robotics, Networking, Artificial intelligence (R.N.A.) Laboratory, in the department of Computer Science, University of Nebraska Omaha. Her research interests include Cyber-Physical Systems, Machine
% Learning, Robotics, and Real-time Computing and Scheduling Algorithms.
% \end{IEEEbiography}
% \vspace{-2.5em}

==> tex/analysis.tex <==
\section{Analysis of the Verification Methods Adopted by DL and its Problems}








==> tex/applicationsbackup.tex <==

\section{Recent works}\label{sec:}


\subsection{Marai et al. \cite{Marai2021-mo}}
Marai et al. \cite{Marai2021-mo} introduced a Digital Twin Box (DTB) model, which is comprised of various devices and sensors, such as a 360-degree camera, GPS, and weather-sensing sensors. The purpose of the DTB model is to control and surveil road infrastructure. It can be developed using a single onboarded computer (SOC), like a Raspberry Pi or Jetson TX2. DTBs have the ability to detect objects and faces from live-streamed video and create profiles based on detected number plates and faces. Additionally, DTBs can collect weather-related information, such as humidity and temperature, through their sensors.

Rather than fully developing the proposed model, the authors focused on detecting objects and faces from a video using the Jetson TX2 device. For object detection, they utilized a single\-shot detector (SSD) \cite{SSD} model, which is faster than YOLO \cite{YOLO} and Faster R-CNN. To detect faces, they employed the face\_recognition library, which is built on deep learning models. After detecting objects and faces and gathering weather data, the DTB creates a profile in the SOC for each unique object and face. The collected information is then sent to a server for further processing.

\textbf{Use cases:} DTBs can be applied to create digital twin roads, with the gathered data being used to enhance the performance of self-driving cars. As DTBs can identify faces and car number plates, they could be employed for national security purposes, such as detecting suspicious activity involving vehicles or individuals. Furthermore, DTBs may be used to determine the cause of road accidents, helping to uncover the actual factors that led to the incident.

\textbf{Cons:} Although the authors proposed using a 360-degree camera, they conducted their object and face detection experiments on 512x512 resolution video. As a result, it is unclear whether the proposed model will work effectively with 360-degree videos.

\textbf{Research direction:} The current work employs SSD for object detection and the face\_recognition library for face detection. However, future research should investigate models that can simultaneously perform object and face detection, potentially improving the efficiency and effectiveness of the DTB system.

In summary, a digital twin is a real-time virtual replica of a physical asset in the digital space that imitates the asset's behavior, performance, and structure \cite{Marai2021-mo}. The primary goal of this technology is to enable continuous monitoring, analysis, testing, and optimization of the physical asset throughout its lifespan.

\subsection{Zhou et al. \cite{9827592}}
    The Building Information Modelling/Model (BIM) is the digital model of a building, and the use cases of the BIM in the Architecture, Engineering, Construction, Operation, and Management (AECOM) have increased a lot. BIM faces synchronizing issues when the physical environment changes. On the other hand, Building Digital Twin (BDT) has been used to sense the condition of the physical environment using the help of the Internet of Things (IoT) for O\&M. Zhou et al. \cite{9827592} propose a model to use the CCTV videos for extending the BIM models toward BDT. But it is challenging to synchronize the digital models with the physical building due to different dimensions, coordinate systems, and object inconsistency. The authors take an approach to utilize Computer Vision (CV) approach to improve the BIM to BDTs. Their CV-based models work in three steps. Firstly the model detects the objects from the live feeds video using the YOLOv5 \cite{YOLOv5}, and secondly detects the position as well as the rotation using the MLP \cite{MLP}. Finally, the camera-BIM location transformation algorithm is used to locate the 3D position of the objects in BIM, and cold-start and run-time object matching schemes are used to sync the detected objects and BIM objects. Besides that, the use of a vanishing point to transform the camera position into the BIM position. Furthermore, they evaluate their model in an office to test the performance of their model in a real-world scenario. They claim that this is the first CV-based approach to utilize both the camera and BIM model to build the BDT. 
    
    \textbf{Research Direction: } In the future, we should focus on detecting 3D objects and textures using sophisticated algorithms or 3D cameras. 

    \textbf{What is DT: } Digital Twins (DTs) are created by combining the digital and physical worlds into one cohesive environment. This means that a DT is a digital representation that mirrors a physical object and is always being updated to reflect any changes made to the physical object.
        
    \textbf{Related Information: } Convolutional neural networks (CNN) are commonly used for detecting objects. There are two types of CNN techniques: one-stage and two-stage. One-stage methods are faster and better for real-time object detection, while two-stage methods are more accurate. Some popular examples of these methods include YOLO, SSD, RetinaNet, Faster R-CNN, Mask R-CNN, and Cascade R-CNN.





\subsection{Melesse et al. \cite{Melesse2022-wm}}
    Inefficient fruit quality monitoring technology within the food supply chain results in significant wastage of fruits. To address this issue, Melesse et al. \cite{Melesse2022-wm} propose a machine learning-based digit twin (DT) for monitoring banana fruit quality using thermal imaging. The proposed solution for monitoring fruit quality during storage comprises an IoT edge layer and an IoT cloud service layer. The IoT edge layer connects thermal cameras and IoT cloud services via a WiFi gateway and an MQTT message broker. Meanwhile, the IoT cloud service layer offers various business services and capabilities for multiple use cases, including supply chain, product, and service management. To establish the connection between IoT sources and cloud services, SAP Edge Services Cloud Edition will be utilized, and pictures from the network of thermal cameras will be stored in SAP Document Services. SAP Intelligent Service will be responsible for image classification using CNN and quality prediction of every fruit during storage. At the same time, SAP Asset Intelligent Network will collect forecast data, monitor the fruit's digital replica, and notify end-users. To facilitate end-user decision-making processes, a custom responsive web application called FooDT client - Retailer Front-End will display the SAP Asset Intelligent Network notification in a user-friendly format. The architecture aims to reduce fruit wastage in the food supply chain by providing accurate and timely information to end-users to enable them to take prompt action and save the product from potential loss. 

    \textbf{Research Direction: } In order to improve the accuracy and reliability of thermal imaging systems for detecting defects in fruits, future research could focus on developing systems that are more robust to environmental variations, such as changes in temperature and humidity. This could be achieved by developing new image processing techniques, machine learning algorithms that can compensate for environmental variations or new hardware and sensors that are less affected by environmental changes. Furthermore, further research could be conducted to explore the feasibility of further combining thermal imaging with other technologies, such as hyperspectral imaging, to improve fruit defect detection's accuracy and reliability.

\subsection{Subramanian et al. \cite{Subramanian2022-gt}}
The study of Subramanian et al. \cite{Subramanian2022-gt} offers an innovative digital twin model that leverages a web camera to obtain facial expressions and discern emotions instantly. The document addresses issues in emotional recognition systems and suggests a strategy to develop a comprehensive dataset for ten distinct emotions, employing body postures to collect images. The MediaPipe framework \cite{mediapipe}  is employed for detecting and drawing features from images for emotion identification. MediaPipe framework aims to offer a cross-functional solution for constructing complex and effective multimedia data processing pipelines. In particular, MediaPipe allows developers to establish pipelines for tasks like object detection, facial recognition, hand tracking, and augmented reality. This framework fuses three faces, hand, and body pose detection models, extracting 543 landmark key points. These coordinates are preserved in a CSV file format, facilitating rapid training by transmitting them to the machine learning algorithm for emotion categorization. The document underlines the efficacy and cost-efficiency of the MediaPipe framework in detecting and extracting features, rendering it an apt solution for real-time image classification tasks. The proposed technique has potential applications in customized healthcare, including real-time monitoring of patient's emotional well-being and offering therapy feedback during psychotherapy sessions. The suggested method has undergone evaluation using various performance metrics, revealing promising outcomes in real-time emotion recognition.

\textbf{Research Direction: } Future research should aim to improve emotion detection accuracy by integrating speech recognition with facial and body emotion detection. This can potentially lead to more robust and comprehensive emotion recognition systems.

    
\subsection{Pengnoo et al. \cite{Pengnoo_9121234}}
Pengnoo et al. \cite{Pengnoo_9121234} propose a Terahertz (THz) signal guidance system for indoor environments that relies on a Digital Twin for modeling, predicting, and controlling signal propagation. The system includes a Controller, Base Station, and Metasurface reflector. This device captures and sends images to the Controller server using two cameras. The researchers employ a machine learning algorithm YOLO, to detect the obstacles and object profiling, as well as a DL algorithm for classifying material types. YOLO enables rapid, real-time obstacle detection and multiple object detection while the Deep Learning algorithm calculates the reflective index for THz signals. This leads to precise obstacle detection and classification, allowing the system to find the best THz signal path while avoiding obstacles. The researchers stress the cost-efficiency and effectiveness of image processing-based approaches like YOLO and DL algorithms for obstacle detection and classification. This technology can determine the optimal THz signal path between the base station and a mobile target while considering obstacles and using geometric, path loss, and Terahertz Potential Field (THzPF) models. This proposed solution can maintain a stable signal connection while reducing the need for antenna and reflector strips. This dynamic control system combines image processing with base station configuration and is appropriate for indoor THz signal guidance.

\textbf{Future research} could explore incorporating YOLO and Deep Learning algorithms in outdoor settings. While the current system focuses on indoor spaces, outdoor environments present unique challenges, such as changing weather and lighting conditions, as well as natural obstacles like trees and foliage. Adapting YOLO and Deep Learning algorithms for outdoor environments could address these challenges by adjusting the YOLO algorithm for varying light conditions and natural barriers and extending the Deep Learning algorithm to account for the impact of material properties on THz signals in outdoor settings.

Additionally, future research might investigate the integration of other sensing modalities, like LiDAR and radar, to improve the accuracy of obstacle detection and classification. By combining YOLO and Deep Learning with other sensing modalities, future systems may achieve even greater precision and efficiency in detecting and classifying obstacles in outdoor environments.

In summary, integrating YOLO and Deep Learning algorithms in outdoor settings represents an exciting and crucial research direction that has the potential to advance THz signal guidance systems and their applications across a wide range of industries and contexts.

% %%%%%%%%%%%%

\subsection{Wang et al. \cite{Wang2021}}
    The optical flow method extracts temporal information from videos by calculating pixel positions' changing distance and direction between adjacent frames. However, the traditional two-stream network, which employs optical flow for feature extraction, is computationally expensive and unsuitable for human-machine interaction (HMI) applications, where real-time responsiveness is crucial.
    
    To address this issue, Wang et al. \cite{Wang2021} propose using 3D-VGG and 3D-ResNet models based on 3D Convolutional Neural Networks (3DCNN) \cite{Ji2013-ay}. These models utilize three-dimensional convolution kernels to extract spatial and temporal features simultaneously, resulting in more efficient data analysis for HMI problems. The 3D-VGG model is an adaptation of the VGG model, initially designed for two-dimensional image classification tasks. The model retains the VGG structure but modifies the input size, number of channels, and convolution kernels for three-dimensional data. The 3D-ResNet model is based on the ResNet architecture, which introduces a residual block to address training difficulties in deep networks. The model uses a three-dimensional input and modifies the convolution blocks and pooling layers accordingly.
    
    The authors aim to enhance human-machine collaboration in digital twin (DT) technology by incorporating 3D-VGG and 3D-ResNet models, prioritizing real-time performance. These models analyze visual information and transform it into action or skeleton data to guide human-machine interaction, generating human skeletal data from video and facilitating better collaboration in virtual environments.


    %%%%%%
    \textbf{Research Direction:} Future research should work on overcoming limitations and making 3D-VGG and 3D-ResNet models better for use in human-machine interaction scenarios with digital twins.

    \textbf{Brief history of the DT: }
    Brief history of the DT: In 2003, Grieves and his team first talked about the idea of a digital twin, but not many people paid attention to it because technology wasn't advanced enough back then \cite{grieves2014}. A digital twin is like a mix of real and virtual things and their connections. In 2011, the Air Force Research Laboratory and NASA worked together to suggest a digital twin for future airplanes, which they described as a highly connected, multi-physical field, multi-scale, and multi-probability simulation model for aircraft. This idea made the digital twin concept more popular.
    
    Many researchers have helped improve the digital twin concept through their studies. For example, Gabor and others thought that digital twins should have expert knowledge for better simulations \cite{Gabor2016ASA}. Rios believed that digital twins should be useful for complex products like airplanes and simpler products too \cite{Ros2016}. Most digital twin research is about digital twin models, connecting the real world with digital things, and how digital twins work together. Researchers study the basic structure and process of making digital twin models \cite{Schroeder2016, Moreno2016}. These models have been used in areas like production systems \cite{Delbrgger2019}, smart factories \cite{Park2019}, and predicting when machines need repairs \cite{Aivaliotis2019, Wang2020}. In these areas, researchers have made progress in understanding how things behave in the real world \cite{Majumdar2013} and testing materials without breaking them \cite{ScottEmuakpor2014MaterialPD}. These advances help figure out model parameters, create behavior rules, and see if the model is accurate.
 
\subsection{Lee et al. \cite{Lee2020}}

Digital twin (DT) is increasingly being utilized due to its significant capacity to bridge the gap between the physical and digital worlds. As per a Grand View Research, Inc. report, the worldwide DT market is expected to achieve a worth of \$26.07 billion by 2025, with a Compound Annual Growth Rate of 38.2\% \cite{Lee2020}.


\subsection{Alexopoulos et al. \cite{Alexopoulos2020}} Alexopoulos et al. \cite{Alexopoulos2020} suggest a new framework that combines Digital Twin technology, Machine Learning, and Transfer Learning to bring AI applications to manufacturing systems. This framework aims to move from traditional automation to smart and adaptable manufacturing. Digital Twins help create and label datasets for Machine Learning models, using both virtual and real-world data for accurate representation and real-time AI decision-making.

The framework uses a layered architecture based on RAMI4.0 \cite{Tuncel2012} with two main parts: the manufacturing system and the Digital Twin. The manufacturing system includes physical components and layers for data processing and AI deployment. In the Digital Twin, virtual models are created using special tools and are combined with real-world data for Machine Learning model training.

Data comes from virtual models, IoT devices, cameras, and machines. The framework manages this data, creates labeled training datasets, and develops Machine Learning models, which are then placed on edge devices for real-time AI decision-making. The Machine Learning models mainly use images from the Digital Twin for training, and the Digital Twin is updated with real-world and virtual data. Once trained, the models help make AI-driven decisions using images and data from the physical world.

A use case shows a camera-based AI service helping a robot detect and handle parts with different orientations in a production environment. A Digital Twin model is created, and synthetic images are used to train a Convolution Neural Network to classify and recognize part orientation. This approach overcomes the time and effort needed for traditional training methods.

In this use case, training datasets come from hundreds of virtual snapshots. These datasets improve an existing Convolution Neural Network model, which is then used for real-time part recognition in a robot control application. Transfer Learning helps enhance the model and apply its recognition capabilities to other parts.

In conclusion, the framework demonstrates the potential of combining virtual and real-world data using Digital Twins for effective Machine Learning model training. This holds promise for future applications focusing on deep learning and Machine Learning models.

\textbf{Research direction: } Future research should explore different use cases to prove the effectiveness of Machine Learning development with Digital Twins. This research should also include advances in data acquisition, simulation, and platform technologies, enabling the integration of Digital Twin-driven Machine Learning models across various production levels, such as devices, stations, lines, and plants.

\textbf{Information related to synthetic image: } Synthetic images are essential in training machine learning algorithms, particularly in image recognition. They aid in training models such as Convolutional Neural Networks (CNNs) \cite{6252468} and Deep Neural Networks (DNNs) \cite{7864335} to identify anomalies and perform image classification. Producing virtual datasets with simulation tools provides a cost-effective and time-saving solution to acquiring and labeling real-world data \cite{7780839, 180406516}. Techniques like domain randomization \cite{8202133} enable neural networks to learn essential features by modifying aspects like illumination and object textures. Synthetic datasets have demonstrated success in tasks like defect detection in manufacturing processes \cite{Dahmen2019}. In summary, synthetic images and virtual environments are valuable assets for training and testing machine learning models in various use cases, including the manufacturing industry.


\subsection{Wu et al. \cite{1011453571734}} This paper proposes an intelligent framework for small surface defect detection in manufacturing processes, incorporating an Edge-Cloud architecture and a deep learning-based algorithm that utilizes advanced image processing techniques. The proposed algorithm utilizes Swin-T as the backbone network to extract features from both color and depth image data. To enhance detection performance, the authors fuse information from both modalities. The algorithm follows a Faster-RCNN structure with three stages: feature extraction, detection, and post-processing. A novel morphological alignment algorithm is also proposed to eliminate false detections and boost precision.

Wu et al. \cite{1011453571734} utilize color images, which provide richer visual information, and process them through a series of steps, including ROI (Region of Interest) proposal, ROI classification and regression, and post-processing via morphological operations. The proposed ROI proposal algorithm segments the input image into multiple candidate regions that may contain defects. In contrast, the ROI classification and regression algorithms determine the probability of the candidate regions being defects and the precise location of the defects, respectively. Finally, the morphological operations are used for post-processing to eliminate false detections and improve the overall accuracy of the algorithm.

In addition, the authors adopt the K-means algorithm to improve anchor box settings for higher accuracy. The algorithm partitions the feature map generated by the backbone network into clusters, and the resulting clusters are used to determine the anchor boxes, which are used to predict the locations of defects. The use of anchor boxes significantly improves the algorithm's accuracy, especially for small defects.

Overall, the proposed algorithm and image processing techniques enable the accurate detection of minor surface defects in manufacturing processes, promoting overall improvement in product quality. The effectiveness of the proposed framework is demonstrated through experiments on two datasets collected from a factory, showcasing the potential of the proposed model for practical applications in intelligent manufacturing.

\subsection{Mukhopadhyay et al. \cite{Mukhopadhyay2022}}
There is a trend to use the machine learning model in the digital environment. Exceptionally, Mukhopadhyay et al. \cite{Mukhopadhyay2022} propose a system where they utilize both physical and digital environments to use the DL model. Their research aims to predict the distance among individuals in close spaces like the office. So, they set up an environment in the office and detected the people using the YOLOv3 models. After detecting the faces in the physical environment, they send the data to the virtual environment to train the model and to predict the distance among the individuals. Then, the digital twin generates the synthetic data in the VR environment to train the model. They use the CNN model to detect the people and office environment in the digital environment. Their model in the virtual environment can detect the people and calculate this distance among the people in the office space. They also leverage the humidity and temperature sensors to control the weather of the office environment from the virtual environment. Their systems help to calculate the distance between each other in the VR environment, which helps to preserve the social distance and safety of the office. 


\textbf{Research direction: } In the future, we may utilize advanced algorithms like Bertoni\textquotesingle s monocular 3D localization algorithm to measure the 3D distance. 


\textbf{Related information for YOLO} Studies have compared the accuracy and processing speed of several object detection models, including YOLOv3, Faster RCNN, Mask RCNN, SSD, and RetinaNet. The results, as reported in references \cite{Mukhopadhyay2019, Punn2020}, demonstrate that YOLOv3 generally outperforms the other models. Additionally, Redmon et al. \cite{YOLO} found that YOLOv3 performs better than other models when fine-tuned with artwork images and tested on a synthetic dataset. These findings indicate that YOLOv3 is an effective and versatile choice for object detection tasks.

\subsection{Jeong et al. \cite{Jeong2022}} Jeong et al. \cite{Jeong2022} work explores using synthetic images to train the deep learning model. After training their model on the images captured from the digital twin, they test the performance on both real and abnormal data. Their proposed model shows that virtually created images can improve the model's accuracy. Mainly their proposed model is based on the digital twin. They create the depth of the damaged tool in the digital environment, capture the images, and convert them into 2D RGB images. Moreover, they also remove the walls using the hue value transformation technique to improve the data quality. Finally, they retrain their model on the generated images using the YOLO v3 deep learning model. The precision value of the model trained on 2D RGB images is only 92.5\%, where the value is 100\% in the case of model training on both normal and abnormal cutting tool data. So, this could improve the performance of the deep learning model by training them on the artificially created image in the digital twin. 

\textbf{Research direction: } In the future, we may explore developing a monitoring system detecting cutting tool damage in real-time and retraining the model. 


\subsection{Mukhopadhyay et al. \cite{Mukhopadhyay9781450390408}} 
It is challenging for many reasons to generate, process, and label the image data from the physical environment. Capturing the actual word data is time-consuming, costly, and sometimes infeasible due to security, privacy, or civic rules. In that case, synthetic data comes handy to train the ML models. Mukhopadhyay et al. \cite{Mukhopadhyay9781450390408} check the feasibility of generating synthetic images in the virtual environment, train them on CNN models and then cross-validate the dataset with real images. After recording the short videos from the physical environment, they send them to the virtual environment. They use the Probuilder tools to simulate the workspace layout and then utilize Physically Based Rendering (PBR) and baked Global Illumination to render the materials and lighting. Finally, they generate two synthetic image datasets in the DT, where one considers ray tracing to check the effect of light on the dataset and uses the Path Tracing algorithms to generate the images using the ray tracing technique. So, their final image dataset is classified into three categories, real images, synthetic images without ray tracking, and with ray tracing. They use the YOLOv3 model to test their dataset, which is pre-train on Open Images Dataset V4. To check the performance of their model, they do case studies on real workspaces and road environments of Indian with usual traffic participants. They also change the person's light, posture condition, and occlusion to validate the performance of the synthetic data. They show that the performance of the CNN-based model for detecting the object from the synthetic images is better than the real data. However, object detection accuracy is lower on ray-tracing images than on images without ray-tracing synthetic images. The accuracy proposed model can detect the object on real word images with 96.044\% accuracy, whereas the accuracy on the synthetic images without ray tracing is 96.981\%. The result shows that we may leverage the synthetic images to train or test the ML models as well as to build the digital twin. 

\textbf{Related information: } Severals games engines bases tool are currently available to generate the synthetic image-based dataset. The perception package \cite{unity-perception2022} of Unity is one of them. According to Jhang et al. \cite{jhang2020training}, the performance of this package for objects with complex orientations, configurations, and lighting conditions are better than the real images. 

Microsoft AirSim \cite{airsim2017fsr} is another tool designed to test and assess drones and autonomous vehicles in virtual environments. Now it can be used to create synthetic datasets for training computer vision models.

UnrealROX \cite{martinez2019unrealrox} is another tool built on top of the Unreal engine, and it can create photorealistic synthetic datasets for robotic vision researchers. It can simulate various indoor robotic activities, including object interactions and poses.


\begin{table*}[htbp]
  \captionsetup{width=1\textwidth}
  \caption{Recent works in image-based digital twins and deep learning models}
  \label{tab:example}
  \centering
   \begin{tabular}{|*{5}{p{3cm}|}}
    \hline
    
    \textbf{Ref} & \textbf{Application} & \textbf{Sensors} & \textbf{ML Model} & \textbf{DT Objective} \\
    \hline
    Ferdousi et al. \cite{Ferdousi101109CASE4999720229926529} & Defect Detection in Rail & Humidity, Positioning, Camera, Stereo Video Recorder, Radar, Drone, LIDAR & CNN & Defect detection in railway \\ \hline

    YI et al. \cite{YI2022552} & Human-Robot Interaction & Color Camera, IR Projector, IR Camera, Kinect v2.0 Camera & CNN & Control the robot \\ \hline

    Melesse et al. \cite{Melesse2022-wm} & Fruit Quality Monitoring & Thermal Camera & CNN & Notify end users \\ \hline

   Alexopoulos et al. \cite{Alexopoulos2020} & AI in Manufacturing & Camera & Inception-v3 CNN model, TensorFlow & Automatic data labeling \\ \hline

   Wu et al. \cite{1011453571734} & Defect Detection in Manufacturing & 2D Camera and 3D Scanner &  Faster-RCNN \cite{Faster_R-CNN}, and Swin-T \cite{swin} based deep learning model & Detect defected product, send notification \\ \hline

    Pengnoo et al. \cite{Pengnoo_9121234} & Networking & Two Cameras, Base Station, Reflector & Python simulation, YOLO & Control antenna and reflector \\ \hline


    Mukhopadhyay et al. \cite{Mukhopadhyay2022} & Workplace Safety using VR & Camera, Temperature and Humidity Sensors & CNN, YOLOv3 & Monitor social distance \\ \hline


    Mukhopadhyay et al. \cite{Mukhopadhyay3489849} & Workplace Safety & Camera & YOLOv3 & Monitor the postures distance in DT \\ \hline



    Jeong et al. \cite{Jeong2022} & Tool Damage Monitoring & Depth Camera & 2D RGB images from synthetic depth maps, YOLOv3 & Monitor tool breakage \\ \hline

    Mukhopadhyay et al. \cite{Mukhopadhyay9781450390408} & Image Processing & Camera & YOLOv3 & Improving object detection performance using synthetic data \\ \hline
    
    
    Zhou et al. \cite{9827592} & Construction Engineering & Monocular Camera & YOLOv5, MLP, Camera-BIM algorithm & Operations \& Maintenance (O\&M) \\ \hline
    
    
    Subramanian et al. \cite{Subramanian2022-gt} & Healthcare & Web Camera & MediaPipe, ML algorithms for classification & Patient Emotions detection \\ \hline
    

    
    Wang et al. \cite{Wang2021} & Human-Machine Interaction & Camera & 3D-VGG and 3D Resnet & Skeletal data from videos and real-time analysis with 3D models. \\ \hline
    


    Marai et al. \cite{Marai2021-mo} & Roads Infrastructure Surveillance & 360° Camera, GPS, Temperature, Humidity, Air Quality Sensors & SSD, Face\_recognition Python library, Google AI Vision API & Data stored locally, sent to OpenStack servers, enabling road monitoring. \\ \hline

  \end{tabular}
\end{table*}


\subsection{Ferdousi et al. \cite{Ferdousi101109CASE4999720229926529}}
 Ferdousi et al. \cite{Ferdousi101109CASE4999720229926529} focus on creating a conceptualized framework called RailTwin to implement Digital Twin (DT) technology in the railway industry. The goal is to improve railway operations and maintenance through AI technologies.

The physical and digital environment is created by establishing two dimensions: the physical space, which involves assets, environment, infrastructure, and processes, and the virtual space, which hosts digital twins of the assets. Continuous bi-directional communication between these dimensions is maintained via a connected vehicle network that enables vehicle-to-vehicle, vehicle-to-cloud, and cloud-to-vehicle communication.

Various sensors are used to collect data from the physical space, including humidity, positioning, camera, stereo video recorder, radar, drone, and LIDAR. Data is collected from two groups: vehicle-side data and track-side data. The AI-inferencing process relies on pre-processed data and includes machine learning, deep learning, transfer learning, reinforcement learning, and explainable AI. 

This data is then pre-processed through cleaning, standardization, labeling, and augmentation before being stored in a database. Next, the AI-inference process, specifically a CNN, analyzes the data and recognizes image features. The CNN model scans the image array, performs convolution, and connects the layers to predict defects. Finally, the Local Interpretable Model Agnostic Explanations(LIME) is applied after the output layer to interpret the prediction. This algorithm modifies data points based on feature values and splits the image outputs into superpixels with similar visual features, such as color or brightness. The use case for this framework involves detecting defects in railway assets using the RailTwin framework and automating the inspection process for improved reliability and sustainability.

\subsection{YI et al. \cite{YI2022552}} YI et al. \cite{YI2022552} develop a user-friendly and safe human-robot collaboration system for smart manufacturing to track human and robot movements in three dimensions accurately so that humans and robots can collaborate in the workspace efficiently and avoid collision.

The physical system consists of a human-robot interface with modules for data collection, human-body structure recognition, and collision prevention. Depth cameras, like Kinect v2.0, capture depth images, which are then processed for noise reduction, resizing, and object detection, sending the information to the digital twin system. 

The digital system uses \textit{Visual Component®} software and \textit{IEC 61499} function blocks to connect virtual and real-world collaboration spaces via a digital twin. The system runs a Convolutional Neural Network (CNN) model on an Ubuntu 18.04 system in the digital environment, which localizes human subjects and obtains 15 key body points. The digital system simulates human-robot collaboration and prevents collisions using the data. It then sends the resulting adjustments back to the physical system. This enables real-time monitoring of distances between human operators and robots, using depth information-based collision avoidance.


\textbf{Rsearch direction: } We may explore more efficient human-robot collaboration with digital twin systems by controlling the speed during collision avoidance for safety. We may extend the approach to involve multiple workers in an industrial environment. 

\subsection{Mukhopadhyay et al. \cite{Mukhopadhyay3489849}} Mukhopadhyay et al. \cite{Mukhopadhyay3489849} present a solution to enforce social distancing by creating a DT of laboratory space. The authors use Unity 3D game engine and its modeling tool, Probuilder, to design the DT with accurate dimensions and Physically Based Materials (PBR) for generating photorealistic real-life materials.

In this study, the data sent to the digital system from the physical environment includes images of the laboratory space captured by the Logitech HD camera. These images contain information about the number of people in the room and their postures.

Furthermore, they implement a Convolutional Neural Network (CNN) model, YOLOv3, for detecting people in real and synthetic datasets. The PyTorch Keypoint RCNN model with a ResNet50 backbone detects key points of the human body to estimate the posture finally. Once the CNN model processes this data, trained on an NVIDIA GeForce RTX 2070 GPU, and detects people and their postures, the digital system maps each person's position and posture to the Digital Twin using virtual humanoids. This mapping allows visualization and generation of analytics related to room occupancy and social distancing without sending any identifiable personal information back to the physical system. The proposed solution achieves 91\% accuracy for real images and 94\% for synthetic images in detecting people. So they got more accuracy on synthetic data. 

\textbf{Related information: } The accuracy of the synthetic image is higher than the real one. 
